Less is KEN: a Universal and Simple Non-Parametric Pruning Algorithm for Large Language Models

Neural network pruning has become increasingly crucial due to the complexity of these models and their widespread use in various fields. Existing pruning algorithms often suffer from limitations such as architecture specificity, excessive complexity and reliance on demanding calculations, rendering them impractical for real-world applications. This paper introduces KEN: a straightforward, universal and unstructured pruning algorithm based on Kernel Density Estimation (KDE). KEN aims to construct optimized transformers by selectively preserving the most significant parameters while restoring others to their pre-training state. This strategy preserves model performance while enabling storage of only the optimized subnetwork, leading to substantial memory savings. Extensive evaluations across seven different LLMs demonstrate that KEN achieves equal or better performance than their original unpruned versions, with a minimum parameter reduction of 25%. Furthermore, in-depth comparisons with established pruning and PEFT algorithms confirm KEN effectiveness. We further introduce KEN$_{viz}$, an explainable tool that visualizes the optimized model composition achieved by KEN from different points of view.

==> sections/tools/comparison_table.tex <==
\begin{table}[htb!]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{lcc}
\hline
Model           & Size                   & \begin{tabular}[c]{@{}c@{}}\texttt{glue-sst2} \\ Accuracy\end{tabular} \\ \hline
Bert-base       & 109M                   & 93.37              \\ \hline
Hybrid          & 94M          & 93.23          \\
HybridNT       & 94M          & 92.20          \\
\textbf{KEN}    & \textbf{80M}           & \textbf{93.80} \\ \hline
Hybrid         & 66M          & 91.97          \\
HybridNT       & 66M          & 90.71          \\
\citet{sajjad2020poor}          & 66M                    & 90.30           \\
\citet{gordon2020compressing}          & 66M                    & 90.80           \\
Flop            & 66M                    & 83.20           \\
\textbf{KEN}    & \textbf{63M}           & \textbf{92.90}  \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Pruning algorithm comparations on SST-2 datasets}
\label{tab: KEN vs Hybrid and other}
\end{table}

==> sections/tools/histogram.tex <==
\makeatletter
\newcommand\resetstackedplots{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(Bert,0) (2,0) (3,0) (4,0) (5,0)};
}
\makeatother

\begin{figure}[htb!]
\centering
\begin{adjustbox}{width=0.95\linewidth}
\begin{tikzpicture}
\begin{axis}[
    reverse legend,
    ybar stacked,
    xtick=data,
    ymin=0,
    xmin = 0.5,
    xmax = 6,
    bar width = 3mm,
    enlarge x limits=0.01,
    ylabel=MegaBytes (MB), font=\small,
    xticklabels={Bert, DistilBERT, DeBERTa, Ernie, Electra},
    x tick label style={font=\small, rotate=20},
    legend style={at={(0.5, -0.2)}, anchor=north, legend columns=2, legend cell align={left}}
]

% Model unpruned
\addplot +[bar shift=-.2cm, color=Original]coordinates {(1, 438) (2,266) (3, 555) (4, 438) (5, 134)};

%Model low compression
\resetstackedplots
\addplot +[bar shift=.15cm, color=LowModel] coordinates {(1, 320) (2, 203) (3, 428) (4, 320) (5, 59.1)};
\addplot +[bar shift=.15cm, LowDictio, fill=LowDictio, postaction={pattern=north east lines}]coordinates {(1,38) (2, 28.4) (3, 48.3) (4, 36.9) (5, 7.91)};

%Model high compression
\resetstackedplots
\addplot  +[bar shift=.5cm, color=HighModel]coordinates {(1, 228) (2, 145) (3, 306) (4, 228) (5, 35.5)};
\addplot  +[bar shift=.5cm, HighDictio, fill=HighDictio, postaction={pattern=north east lines}] coordinates {(1, 32.2) (2, 20) (3, 42.4) (4, 32.3) (5, 7.08)};

\legend{Original file size, 
Low sparsity model file size, Low sparsity supp. dict file size, 
High sparsity model file size, High sparsity supp. dict file size}
\end{axis}
\end{tikzpicture}
\end{adjustbox}
\caption{Comparison of the .pt file size between the original and compressed transformer weights}
\label{fig: Compression histogram}
\end{figure}

